Towards Controllable Time Series Generation

Time Series Generation (TSG) has emerged as a pivotal technique in synthesizing data that accurately mirrors real-world time series, becoming indispensable in numerous applications. Despite significant advancements in TSG, its efficacy frequently hinges on having large training datasets. This dependency presents a substantial challenge in data-scarce scenarios, especially when dealing with rare or unique conditions. To confront these challenges, we explore a new problem of Controllable Time Series Generation (CTSG), aiming to produce synthetic time series that can adapt to various external conditions, thereby tackling the data scarcity issue. In this paper, we propose \textbf{C}ontrollable \textbf{T}ime \textbf{S}eries (\textsf{CTS}), an innovative VAE-agnostic framework tailored for CTSG. A key feature of \textsf{CTS} is that it decouples the mapping process from standard VAE training, enabling precise learning of a complex interplay between latent features and external conditions. Moreover, we develop a comprehensive evaluation scheme for CTSG. Extensive experiments across three real-world time series datasets showcase \textsf{CTS}'s exceptional capabilities in generating high-quality, controllable outputs. This underscores its adeptness in seamlessly integrating latent features with external conditions. Extending \textsf{CTS} to the image domain highlights its remarkable potential for explainability and further reinforces its versatility across different modalities.

==> tables/ablation_fidelity.tex <==
\begin{table}[t]
\centering
\captionsetup{skip=0.5em}
\small
\setlength\tabcolsep{5pt}
\caption{Ablation study of generation fidelity.}
\label{tab:ablation-fidelity}%
\resizebox{\columnwidth}{!}{%
  \begin{tabular}{ccccccccc} \toprule
  \multirow{2.5}[6]{*}{\textbf{Methods}} & \multicolumn{4}{c}{\textbf{Air-SZ}} & \multicolumn{4}{c}{\textbf{Boiler}} \\
  \cmidrule(lr){2-5}\cmidrule(lr){6-9} & \multicolumn{2}{c}{\textbf{Interp.}} & \multicolumn{2}{c}{\textbf{Extrap.}} & \multicolumn{2}{c}{\textbf{Interp.}} & \multicolumn{2}{c}{\textbf{Extrap.}} \\
  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} & \textbf{ED$\downarrow$} & \textbf{DTW$\downarrow$} & \textbf{ED$\downarrow$} & \textbf{DTW$\downarrow$} & \textbf{ED$\downarrow$} & \textbf{DTW$\downarrow$} & \textbf{ED$\downarrow$} & \textbf{DTW$\downarrow$} \\
  \midrule
  \textsf{CTS}  &  &  &  &  &  &  &  &   \\
  \textsf{CTS$-$NNS} &  &  &  &  &  &  &  &   \\
  \textsf{CTS$-$DCS} &  &  &  &  &  &  &  &   \\
  \textsf{CTS$-$NNS$-$DCS} &  &  &  &  &  &  &  &   \\
  \bottomrule
  \end{tabular}%
}  
\end{table}%



==> tables/ablation_perceptual.tex <==
\begin{table}[t]
\centering
\captionsetup{skip=0.5em}
\small
\setlength\tabcolsep{3pt}
\caption{Ablation study of perceptual similarity.}
\label{tab:ablation-perceptual}%
\resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccccccc} \toprule
  \multirow{2.5}[6]{*}{\textbf{Methods}} & \multicolumn{4}{c}{\textbf{Air-SZ}}    & \multicolumn{4}{c}{\textbf{Boiler}} \\
  \cmidrule(lr){2-5}\cmidrule(lr){6-9} & \multicolumn{2}{c}{\textbf{Interp.}} & \multicolumn{2}{c}{\textbf{Extrap.}} & \multicolumn{2}{c}{\textbf{Interp.}} & \multicolumn{2}{c}{\textbf{Extrap.}} \\
  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} & \textbf{C-FID$\downarrow$} & \textbf{ACD$\downarrow$} & \textbf{C-FID$\downarrow$} & \textbf{ACD$\downarrow$} & \textbf{C-FID$\downarrow$} & \textbf{ACD$\downarrow$} & \textbf{C-FID$\downarrow$} & \textbf{ACD$\downarrow$} \\
  \midrule
  \textsf{CTS} & 0.838 & \textbf{0.066} & \textbf{14.207} & 0.270 &  &  &  &   \\
  \textsf{CTS$-$NNS} & 0.778 & 0.072 & 23.825 & 0.277 &  &  &  &   \\
  \textsf{CTS$-$DCS} & \textbf{0.585} & 0.069 & 19.475 & \textbf{0.266} &  &  &  &   \\
  \textsf{CTS$-$NNS$-$DCS} & 1.044 & 0.069 & 20.701 & 0.276 &  &  &  &   \\
  \bottomrule
  \end{tabular}
}
\end{table}%



==> tables/datasets.tex <==
\begin{table}[t]
\centering
\captionsetup{skip=0.5em}
\caption{The statistics of three real-world time series datasets.}
\label{tab:dataset}%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
  \toprule
  \textbf{Datasets} & $n$ & $d_r$ & $m$ & \textbf{Test Size} & \textbf{Content} \\ \midrule
  Air-GZ  &         &                 & 4  &        & Air Quality \\
  Air-SZ  & 3,812   & 168 $\times$ 6  & 4  & 424    & Air Quality \\
  Boiler  & 80,935  & 192 $\times$ 11 & 1  & 8,993  & Machine Operations \\
  % Air-BJ  &       &                 & 4  &        & Air Quality \\
  % Air-TJ  & 7,731 & 168 $\times$ 6  & 4  & 860    & Air Quality \\
  \bottomrule
\end{tabular}}
\end{table}


% \textbf{Datasets} & \textbf{\# Training Samples} & \textbf{\# Test Samples} & $\num{\bm{C}}$ & \textbf{Content} \\ \midrule
% dSprites & 500,032 & 50,000 & & & 4   & 2D Shapes  \\
% 3DChairs & 81,344  & 5,022  & & & 2   & 3D Chairs  \\
% Pubfig   & 8,832   & 532    & & & 6   & Human Face \\ % 58,797
% CelebA  & 50,000  & 32 $\times$ 32  & 18 & 10,000 & Human Face \\ % 202,599
% FFHQ    & 61,632  & 32 $\times$ 32  & 8  & 1,033  & Human Face \\ % 70,000
% Teapots & 190,016 & 32 $\times$ 32  & 5  & 9,984  & Edinburgh Teapots \\
  
% Air: 168*6, 6*168
% Boiler: 11*192

==> tables/generalization_test_ts.tex <==
\begin{table}[ht]
\centering
\captionsetup{skip=0.5em}
\setlength\tabcolsep{3pt}
\caption{Generalization test on time series datasets.}
\label{tab:generalization-ts}%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccccccc} \toprule
  \multirow{2}[6]{*}{\textbf{\textsf{CTS} with}} & \multicolumn{6}{c}{\textbf{Interpolation}} & \multicolumn{6}{c}{\textbf{Extrapolation}} \\
  \cmidrule(lr){2-7} \cmidrule(lr){8-13} & \multicolumn{2}{c}{\textbf{Air-GZ}} & \multicolumn{2}{c}{\textbf{Air-SZ}} & \multicolumn{2}{c}{\textbf{Boiler}} & \multicolumn{2}{c}{\textbf{Air-GZ}} & \multicolumn{2}{c}{\textbf{Air-SZ}} & \multicolumn{2}{c}{\textbf{Boiler}} \\
  \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13} & \textbf{ACC$\uparrow$} & \textbf{W-F1$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{W-F1$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{W-F1$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{AUC$\uparrow$}  & \textbf{ACC$\uparrow$} & \textbf{AUC$\uparrow$} & \textbf{ACC$\uparrow$}  & \textbf{AUC$\uparrow$} \\ 
  \midrule
  \textsf{TimeVAE} & & & 0.758 & 0.751 & 0.517 & 0.474 & &  & 0.906 & 0.750 & 0.581 &  0.687 \\
  \textsf{TimeVQVAE} & & & & & & & & & & & & \\ 
  \bottomrule
\end{tabular}%
}
\end{table}


% \begin{table*}[htbp]
% \centering
% \captionsetup{skip=0.5em}
% \small
% \setlength\tabcolsep{3pt}
% \caption{Generalization test on time series datasets.}
% \label{tab:generalization}%
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccccccccccccccccc} \toprule
%   \multirow{2}[6]{*}{\textbf{\textsf{CTS} with}} & \multicolumn{10}{c}{\textbf{Interpolation}} & \multicolumn{10}{c}{\textbf{Extrapolation}} \\
%   \cmidrule(lr){2-11} \cmidrule(lr){12-21} & \multicolumn{2}{c}{\textbf{Air-BJ}} & \multicolumn{2}{c}{\textbf{Air-GZ}} & \multicolumn{2}{c}{\textbf{Air-SZ}} & \multicolumn{2}{c}{\textbf{Air-TJ}} & \multicolumn{2}{c}{\textbf{Boiler}} & \multicolumn{2}{c}{\textbf{Air-BJ}} & \multicolumn{2}{c}{\textbf{Air-GZ}} & \multicolumn{2}{c}{\textbf{Air-SZ}} & \multicolumn{2}{c}{\textbf{Air-TJ}} & \multicolumn{2}{c}{\textbf{Boiler}} \\
%   \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11} \cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}\cmidrule(lr){20-21} & \textbf{ACC$\uparrow$} & \textbf{W-F1$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{W-F1$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{W-F1$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{W-F1$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{W-F1$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{AUC$\uparrow$} & \textbf{ACC$\uparrow$}  & \textbf{AUC$\uparrow$} & \textbf{ACC$\uparrow$} & \textbf{AUC$\uparrow$}  & \textbf{ACC$\uparrow$} & \textbf{AUC$\uparrow$} & \textbf{ACC$\uparrow$}  & \textbf{AUC$\uparrow$} \\ 
%   \midrule
%   \textsf{TimeVAE} & & & & & 0.758 & 0.751 & 0.724 & 0.722 & 0.517 & 0.474 & & & &  & 0.906 & 0.750 & 0.601 & 0.658 & 0.581 &  0.687 \\
%   \textsf{TimeVQVAE} & & & & & & & & & & & & & & & & & & & & \\ 
%   \bottomrule
% \end{tabular}%
% }
% \end{table*}

